DREAM-PCD: Deep Reconstruction and Enhancement of mmWave Radar Pointcloud

Millimeter-wave (mmWave) radar pointcloud offers attractive potential for 3D sensing, thanks to its robustness in challenging conditions such as smoke and low illumination. However, existing methods failed to simultaneously address the three main challenges in mmWave radar pointcloud reconstruction: specular information lost, low angular resolution, and strong interference and noise. In this paper, we propose DREAM-PCD, a novel framework that combines signal processing and deep learning methods into three well-designed components to tackle all three challenges: Non-Coherent Accumulation for dense points, Synthetic Aperture Accumulation for improved angular resolution, and Real-Denoise Multiframe network for noise and interference removal. Moreover, the causal multiframe and "real-denoise" mechanisms in DREAM-PCD significantly enhance the generalization performance. We also introduce RadarEyes, the largest mmWave indoor dataset with over 1,000,000 frames, featuring a unique design incorporating two orthogonal single-chip radars, lidar, and camera, enriching dataset diversity and applications. Experimental results demonstrate that DREAM-PCD surpasses existing methods in reconstruction quality, and exhibits superior generalization and real-time capabilities, enabling high-quality real-time reconstruction of radar pointcloud under various parameters and scenarios. We believe that DREAM-PCD, along with the RadarEyes dataset, will significantly advance mmWave radar perception in future real-world applications.

==> article/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/ruixugeng.jpg}}]{Ruixu Geng}
   received the B.S. degree from the University of Electronic Science and Technology of China, Chengdu, in 2019, where he is currently pursuing the MS degree with the School of Information and Communication Engineering. His research interests include computational imaging and computer vision.
\end{IEEEbiography}

\vspace{-10 mm} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/yanghu.png}}]{Yang Hu}
   received the B.S. and Ph.D. degrees in electrical engineering from the University of Science and Technology of China, Hefei, China, in 2004 and 2009 respectively. She was with the University of Maryland Institute for Advanced Computer Studies as a research associate from 2010 to 2015. She is currently an associate professor with the School of Information Science and Technology at the University of Science and Technology of China. Her current research interests include computer vision, machine learning and multimedia signal processing.
\end{IEEEbiography}

\vspace{-10 mm} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/zhilu.png}}]{Zhi Lu}
   received the B.S. and M. A. degree from University of Electronic Science and Technology of China, Chengdu, China, in 2015 and 2017 respectively. He is currently pursuing the Ph.D. degree at the School of Information and Communication Engineering, University of Electronic Science and Technology of China. His research interests are in data mining and multimedia.
\end{IEEEbiography}

\vspace{-10 mm} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/congyu.jpg}}]{Cong Yu}
   received B.S. degree from the University of Electronic Science and Technology of China, Chengdu, China, in 2019. He is currently pursuing the Ph.D. degree at the School of Information and Communication Engineering, University of Electronic Science and Technology of China, Chengdu, China. His current research interests include wireless sensing, image synthesis, and adversarial learning.
\end{IEEEbiography}

\vspace{-10 mm} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/houqiangli.jpg}}]{Houqiang Li}
   (S’12, F’21) received the B.S., M.Eng., and Ph.D. degrees in electronic engineering from the University of Science and Technology of China, Hefei, China, in 1992, 1997, and 2000, respectively, where he is currently a Professor with the Department of Electronic Engineering and Information Science. 

   His research interests include image/video coding, image/video analysis, computer vision, reinforcement learning, etc.. He has authored and co-authored over 200 papers in journals and conferences. He is the winner of National Science Funds (NSFC) for Distinguished Young Scientists, the Distinguished Professor of Changjiang Scholars Program of China, and the Leading Scientist of Ten Thousand Talent Program of China. He is the associate editor (AE) of IEEE TMM, and served as the AE of IEEE TCSVT from 2010 to 2013. He served as the General Co-Chair of ICME 2021 and the TPC Co-Chair of VCIP 2010. He is the recipient of National Technological Invention Award of China (second class) in 2019 and the recipient of National Natural Science Award of China (second class) in 2015. He was the recipient of the Best Paper Award for VCIP 2012, the recipient of the Best Paper Award for ICIMCS 2012, and the recipient of the Best Paper Award for ACM MUM in 2011.
\end{IEEEbiography}

\vspace{-10 mm} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/hengyuzhang.jpg}}]{Hengyu Zhang}
   received his Master and PhD degrees from West China Medicine School, Sichuan University, in 1996 and 2010, respectively. He is now a professor in the school and a deputy chief physician of West China Hospital, engaging cardiac pacing, electrophysiology, and pacemaker implantation with international leading level. He was a visiting scientist in School of Medicine, National University of Singapore, from February 2008 to February 2009. He has been Director of West China Syncope Center since 2021, where medical images are heavily involved.
\end{IEEEbiography}

\vspace{-10 mm} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./pic/biography/yanchen.png}}]{Yan Chen}
   (SM'14) received the bachelor degree from the University of Science and Technology of China in 2004, the M.Phil. degree from the Hong Kong University of Science and Technology in 2007, and the Ph.D. degree from the University of Maryland, College Park, MD, USA, in 2011. He was with Origin Wireless Inc. as a Founding Principal Technologist. From Sept. 2015 to Feb. 2020, he was a Professor with the School of Information and Communication Engineering at the University of Electronic Science and Technology of China. He is currently a Professor with the School of Cyber Science and Technology at the University of Science and Technology of China. 

   Dr. Chen’s research interests include multimodal sensing and imaging, multimedia signal processing, and wireless multimedia. He is a co-author of “Reciprocity, Evolution, and Decision Games in Network and Data Science” (Cambridge University Press, 2021) and “Behavior and Evolutionary Dynamics in Crowd Networks: An Evolutionary Game Approach” (Springer, 2020), as well as co-author of over 200 technical papers including more than 100 IEEE journal papers. He is the Associate Editor for IEEE Transactions on Network Science and Engineering, IEEE Transactions on Signal and Information Processing over Networks, and on the Editorial Board for MDPI Sensors. He is the Chair for APSIPA Signal and Information Processing Theory and Methods (SIPTM) Technical Committee, a Distinguished Lecturer for APSIPA, the Secretary-General for the CES Young Scientist Network Multimedia Technical Committee. He is an organizing co-chair of PCM 2017, a special session co-chair of APSIPA ASC 2017, the 10K Best Paper Award Committee member of ICME 2017, the multimedia communications symposium lead chair of WCSP 2019, an Area Chair for ACM Multimedia 2021. He was the recipient of multiple honors and awards, including the best paper award at the APSIPA ASC in 2020, the best student paper award at the PCM in 2017, the best student paper award at the IEEE ICASSP in 2016, the best paper award at the IEEE GLOBECOM in 2013.
\end{IEEEbiography}

